Q-NL Verifier: Leveraging Synthetic Data for Robust Knowledge Graph Question Answering

Question answering (QA) requires accurately aligning user questions with structured queries, a process often limited by the scarcity of high-quality query-natural language (Q-NL) pairs. To overcome this, we present Q-NL Verifier, an approach to generating high-quality synthetic pairs of queries and NL translations. Our approach relies on large language models (LLMs) to generate semantically precise natural language paraphrases of structured queries. Building on these synthetic Q-NL pairs, we introduce a learned verifier component that automatically determines whether a generated paraphrase is semantically equivalent to the original query. Our experiments with the well-known LC-QuAD 2.0 benchmark show that Q-NL Verifier generalizes well to paraphrases from other models and even human-authored translations. Our approach strongly aligns with human judgments across varying query complexities and outperforms existing NLP metrics in assessing semantic correctness. We also integrate the verifier into QA pipelines, showing that verifier-filtered synthetic data has significantly higher quality in terms of translation correctness and enhances NL to Q translation accuracy. Lastly, we release an updated version of the LC-QuAD 2.0 benchmark containing our synthetic Q-NL pairs and verifier scores, offering a new resource for robust and scalable QA.

==> incorrect_example1.tex <==
\begin{wrongbox}
    \textbf{Query} 
    \begin{lstlisting}[basicstyle=\ttfamily\small, frame=none, breaklines=true]
SELECT ?value WHERE { [Zooey Deschanel] [nominated for] ?s . ?s [nominated for] [Primetime Emmy Award for Outstanding Lead Actress in a Comedy Series] . ?s [for work] ?value}
\end{lstlisting}

    \textbf{Translation}\\
For which comedy television series was Zooey Deschanel nominated for a Primetime Emmy Award?
\end{wrongbox}

